Turing LLM Post-Training: Calibrated Distillation and Efficient Dynamic-MoE Execution

We study post-training for dynamically routed mixture-of-experts (MoE) models, focusing on integrating independently optimized specialists while keeping consolidation efficient. Our approach combines calibrated multi-teacher on-policy distillation (C-MOPD), which matches each selected teacher on a local Top-$K$ support with teacher-wise loss normalization and clipping, with an execution path that uses post-capacity bounded-width dispatch, final-route replay, and asynchronous rollout--training overlap. On Turing-20B-A2B, the selected model achieves a four-domain normalized integration score of 0.9988 and retains at least 90.16\% of the measured specialist gain in every domain. At matched $K=32$, the full calibration objective scores 0.9962, compared with 0.9724 without calibration and 0.9834 without clipping. At a matched 8K response cap, the model exceeds both shared SFT and Qwen3-8B on all four reasoning-enabled mathematics and code benchmarks (unweighted mean: 85.92, versus 80.33 for Qwen3-8B and 74.21 for SFT), and improves over SFT on ten of twelve broader evaluation metrics. In a PPU-based profile, the combined execution configuration reduces consolidation step time from 398.7 to 139.3 seconds, an observed 2.86$\times$ speedup over serial execution. These results demonstrate strong specialist integration alongside more efficient consolidation, while reflecting the complete training and execution framework rather than any single component.

==> sec/2_related_works.tex <==
% !TeX root = ../main.tex
\section{Related Work}

\subsection{Multi-Stage and Multi-Domain Post-Training}

RL with verifiable rewards is widely used to improve mathematics, code, instruction following, and tool use. DeepSeek-R1 combines cold-start supervision with large-scale RL, while executable feedback provides direct correctness signals for code generation~\cite{deepseekr1,rltf}. GSPO uses sequence-level importance weighting and clipping to stabilize policy optimization, particularly for MoE policies~\cite{gspo}. Multi-domain training introduces an additional allocation problem: M2RL shows that interference depends on the task mixture rather than affecting every domain uniformly~\cite{m2rl}. These findings motivate domain-specific sampling and verifier design, but they do not determine whether specialist capabilities should be integrated by mixed RL, sequential RL, or distillation. The present results characterize a specialize-then-consolidate route; they do not establish that it is intrinsically superior to those alternatives.

Rejection-sampling fine-tuning and teacher correction can strengthen the shared initialization before RL~\cite{yuan2023rft}. Prompt-controlled reasoning-enabled and direct-response examples also broaden interface coverage~\cite{qwen3,katv1}. Our framework uses these established techniques to construct the common starting point for specialist learning; C-MOPD provides the subsequent consolidation mechanism.

\subsection{Multi-Teacher On-Policy Distillation}

Offline distillation supervises fixed teacher trajectories and can miss prefixes induced by student errors. GKD queries teachers on student-generated sequences, MiniLLM optimizes sequence-level reverse KL, and DistiLLM combines alternative divergences with adaptive replay~\cite{gkd,minillm,distillm}. Recent analyses of sampled-token OPD motivate matching a teacher's Top-$K$ local support instead of relying on one sampled action~\cite{revisitingopd}. MOPD routes domain data to specialist teachers and reports stronger capability integration than mixed RL, cascade RL, and offline fine-tuning; D3-MOPD further adapts domain sampling to heterogeneous convergence rates~\cite{mopd,d3mopd}.

Our algorithm operates in this setting but targets a different failure mode: heterogeneous teacher losses may remain numerically imbalanced even when data routing is appropriate. \methodname combines local-support reverse KL with teacher-wise scale control, token-level clipping, and explicit weights. The fixed-support objective comparisons in \autoref{sec:calibration-analysis} separate the available evidence for scale normalization and clipping from support-size selection; on-policy generation, teacher routing, and Top-$K$ matching are inherited ingredients.

\subsection{Efficient Post-Training for Dynamic MoE}

Fixed-Top-$k$ routing chooses input-dependent expert identities but gives every token the same expert count. Quantile Routing relaxes this count constraint using expert-specific thresholds and a controlled average budget~\cite{turingllm}. Its pretraining benefits are evaluated in the TuringLLM report; we retain this router during post-training.

Switch Transformer motivates fixed Top-1 routing through simpler implementation and reduced routing computation and communication~\cite{switchtransformer}. Other open-source work supports token-adaptive allocation under different training settings. Dynamic MoE uses confidence-based expert selection and reports an average benchmark improvement of 0.7 points over Top-2 routing with less than 90\% of the baseline's activated parameters~\cite{dynamicmoe}. AdaMoE adds zero-computation null experts so that the number of real experts can vary; when fine-tuning Mixtral-8x7B on ARC-C, it reports 14.5\% fewer FLOPs and 1.69 points higher accuracy~\cite{adamoe}. Both release code. These results motivate preserving dynamic allocation, but do not establish universal superiority across architectures or imply proportional wall-clock speedups.

Execution efficiency is a separate issue. MegaBlocks identifies the token-dropping versus padding trade-off and uses block-sparse kernels to support dropless MoE execution~\cite{megablocks}. Capacity-Aware Inference identifies overloaded experts as latency-determining stragglers under expert parallelism~\cite{capacityaware}. These issues also affect fixed-$k$ routing; variable-$k$ adds a variable per-token fan-out. Our RL-stage adaptation bounds this fan-out after capacity filtering while preserving all non-overflow assignments; it builds on the base model's dynamic router rather than replacing its expert-selection rule. It complements, rather than replaces, efficient sparse kernels and expert-load balancing.

Distributed post-training systems separate high-throughput rollout generation from memory-intensive policy optimization. HybridFlow/veRL formalizes flexible RLHF dataflows and placement; slime connects Megatron training with SGLang generation; AReaL and AsyncFlow overlap rollout and optimization while managing policy staleness~\cite{hybridflow,slime,areal,asyncflow}. MoE policies add a route-consistency requirement because rollout and actor engines can select different experts for the same token. R3 records the inference route and replays it during training~\cite{r3}. We use this alignment contract with the final capacity- and width-processed route. Within our framework, these mechanisms support C-MOPD execution rather than define its learning objective. The available profile measures their combined effect in the consolidation workflow and does not isolate every main effect or interaction.

